The Label Complexity of Active Learning from Observational Data

Counterfactual learning from observational data involves learning a classifier on an entire population based on data that is observed conditioned on a selection policy. This work considers this problem in an active setting, where the learner additionally has access to unlabeled examples and can choose to get a subset of these labeled by an oracle. Prior work on this problem uses disagreement-based active learning, along with an importance weighted loss estimator to account for counterfactuals, which leads to a high label complexity. We show how to instead incorporate a more efficient counterfactual risk minimizer into the active learning algorithm. This requires us to modify both the counterfactual risk to make it amenable to active learning, as well as the active learning process to make it amenable to the risk. We provably demonstrate that the result of this is an algorithm which is statistically consistent as well as more label-efficient than prior work.

==> intro.tex <==
\section{Introduction}

Counterfactual learning is an emerging problem that arises naturally in many applications. In this problem, the learner is given observational data -- a set of examples selected according to some policy along with their labels -- as well as access to the policy that selects the data, and the goal is to construct a classifier with high performance on an entire population -- not just on the observational data distribution. An example is learning to predict if a treatment will be effective based on features of a patient. Here, we have some observational data on how the treatment works for patients that were assigned to it, but if the treatment is given only to a certain category of patients, then this data is not reflective of the population. Thus the main challenge in counterfactual learning is how to counteract the effect of the observation policy and build a classifier that applies to the entire population.

This work considers counterfactual learning in the active setting, which has received very recent attention in a few different contexts~\cite{YCJ18, SSSVSK19, AZS18}. In addition to observational data, the learner has an online stream of unlabeled examples drawn from the underlying population distribution, and the ability to selectively label a subset of these in an interactive manner. The learner's goal is to again build a classifier while using as few label queries as possible. The advantage of the active over the passive is its potential for more efficient solutions; the question however is how to do this algorithmically.

% -- it offers an opportunity to correct the sample selection bias present in the observational data through freshly labeled samples, and unlike learning from randomly drawn samples from the population alone, it can exploit observational data. 
%The advantage of active over the passive is that it offers an opportunity to efficiently correct the sample selection bias present in observational data by getting fresh labeled examples in underrepresented regions of the instance space; however, the challenge is how to do this efficiently and while still maintaining statistical consistency.  \kc{basically say that this has to be done carefully. Also bring in randomized control trials}

Prior work in active counterfactual learning~\cite{YCJ18} has used a modified version of disagreement-based active learning, along with an importance weighted empirical risk to account for the counterfactual. However, a problem with this approach is that the importance weighted risk estimator can have extremely high variance when the importance weights -- that reflect the inverse of how frequently an instance in the population is selected by the policy -- are high; this may happen if, for example, certain patients are rarely given the treatment. This high variance in turn can result in high sample requirement for the learner.

Passive counterfactual learning addresses this challenge by minimizing instead a counterfactual risk~\cite{SJ15CRM} -- an importance weighted loss that combines a variance regularizer and importance weight clipping or truncation to achieve low generalization error. This risk however cannot be combined with active learning for two reasons. The first is that the variance regularizer itself is a function of the entire dataset, and is therefore challenging to use in interactive learning where data arrives in batches. The second reason is that the minimizer of the (expected) counterfactual risk depends on $n$, the data set size, which again is inconvenient for learning in an interactive manner. 

In this work, we address both challenges. To address the first, we use, instead of a variance regularizer, a novel regularizer based on the second moment; the advantage is that it decomposes across multiple segments of the data set as which makes it amenable for active learning. We provide generalization bounds for this modified counterfactual risk minimizer, and show that it has almost the same performance as counterfactual risk minimization with a variance regularizer~\cite{SJ15CRM}.

The second challenge arises because disagreement-based active learning ensures statistical consistency by maintaining a set of plausible minimizers of the expected risk. This is problematic when the minimizer of the expected risk itself changes between iterations -- as would happen even with our modified counterfactual risk as the regularizer depends on $n$. We address this challenge by introducing a novel variant of disagreement-based active learning which is always guaranteed to maintain the population risk minimizer in its plausible set. 

To improve sample efficiency, we then propose a third novel component -- a new sampling algorithm for correcting sample selection bias that selectively queries labels of those examples which are underrepresented in the observational data. Combining these three components gives us a new algorithm. We analyze this newly proposed algorithm theoretically, and show that it is statistically consistent -- in the sense that it converges to the true minimizer of the population risk given enough data. Finally, we analyze its label complexity, and demonstrate that it is better than several alternatives -- prior work~\cite{YCJ18} in counterfactual active learning, learning only from observational data, and pure active learning alone.



